Functional reducts of Boolean algebras

In this paper we classify some special reducts of the countable atomless Boolean algebra which we call functional reducts. We prove that there are exactly $13$ such structures up to first order interdefinability.

==> minden_egyutt.tex <==

\begin{tikzpicture}[scale=1, remember picture, shift={(current page.south)}]
\tikzstyle{every node}=[shape=rectangle, draw, fill=white!]
\tikzstyle{white}=[shape=rectangle, draw, fill=white!]
\tikzstyle{green}=[shape=rectangle, draw, fill=white!, font=\large]
\tikzstyle{blue}=[shape=circle, draw, fill=white!]
\tikzstyle{red}=[shape=rectangle, draw, fill=white!]
\tikzstyle{ures}=[shape=circle, draw, fill=white!]


\tikzstyle{k}=[draw=none, fill=none]

\path

(0, 14)  node[k] (100)  {}
(-1, 13)  node[k] (101)  {}
(0, 13)  node[k] (102)  {}
(0, 12)  node[k] (103)  {}
(4, 13)  node[k] (104)  {}
(0, 10)  node[k] (105)  {}
(-6, 9)  node[k] (106)  {}
(-5, 6)  node[k] (107)  {}
(0, 4)  node[k] (108)  {}
(-4 ,9)  node[k] (109)  {}
(-3, 13)  node[k] (110)  {}
(-2, 10)  node[k] (111)  {}
(0, 8)  node[k] (112)  {}
(0,5)  node[k] (113)  {}
(2,5)  node[k] (114)  {}
(4,5)  node[k] (115)  {}
(4,6)  node[k] (116)  {}
(-3, 5)  node[k] (117)  {}
(-3,6)  node[k] (118)  {}
(-1, 6)  node[k] (119)  {}
(0, 9)  node[k] (120)  {}
(1,6)  node[k] (121)  {}
(1,7)  node[k] (122)  {}
(-5, 7)  node[k] (123)  {}
(-3, 7)  node[k] (124)  {}
(-1, 7)  node[k] (125)  {}
(-1, 8)  node[k] (126)  {}
(2, 7)  node[k] (127)  {}
(2,8)  node[k] (128)  {}
(2,10)  node[k] (129)  {}
(4, 9)  node[k] (130)  {}
(4, 10)  node[k] (131)  {}
(4, 12)  node[k] (132)  {}
(2, 13)  node[k] (133)  {}
(2, 12)  node[k] (134)  {}
;
\draw
(115) -- (108)
(114) -- (108)
(113) -- (108)
(117) -- (108)
(116) -- (115)
(121) -- (115)
(116) -- (114)
(119) -- (114)
(116) -- (113)
(118) -- (113)
(112) -- (113)
(121) -- (117)
(119) -- (117)
(118) -- (117)
(107) -- (117)
(122) -- (121)
(125) -- (121)
(122) -- (119)
(124) -- (119)
(122) -- (118)
(123) -- (118)
(120) -- (118)
(106) -- (107)
(109) -- (107)
(123) -- (107)
(124) -- (107)
(125) -- (107)
(132) -- (129)
(122) -- (116)
(126) -- (122)
(128) -- (122)
(131) -- (126)
(126) -- (125)
(126) -- (124)
(126) -- (123)
(111) -- (123)
(120) -- (112)
(111) -- (120)
(129) -- (120)
(127) -- (119)
(130) -- (107)
(132) -- (111)
(110) -- (111)
(110) -- (106)
(101) -- (106)
(110) -- (109)
(102) -- (109)
(100) -- (110)
(128) -- (127)
(130) -- (127)
(129) -- (128)
(131) -- (128)
(105) -- (130)
(131) -- (130)
(132) -- (131)
(134) -- (131)
(104) -- (132)
(103) -- (105)
(134) -- (105)
(101) -- (103)
(102) -- (103)
(133) -- (103)
(133) -- (134)
(104) -- (134)
(100) -- (101)
(100) -- (102)
(100) -- (133)
(100) -- (104)
;
\path
(0, 14)  node[green] (0)  {{$\emptyset$}}
(-1, 13)  node[green] (1)  {{$0$}}
(0, 13)  node[green] (2)  {{$1$}}
(0, 12)  node[green] (3)  {{$0,1$}}
(4, 13)  node[green] (4)  {{$\neg$}}
(0, 10)  node[green] (5)  {{$\neg , 0, 1$}}
(-6, 9)  node[green] (6)  {{$+_0,0$}}
(-5, 6)  node[green] (7)  {{$+_0,0,1$}}
(0, 4)  node[green] (8)  {{$\s ,+_0,0,1$}}
(-4 ,9)  node[green] (9)  {{$ +_1,1$}}
(-3, 13)  node[green] (10)  {{$\Sigma$}}
(-2, 10)  node[green] (11)  {{$\Sigma_1$}}
(0, 8)  node[green] (12)  {{$M$}}
(0,5)  node[blue] (13)  {a}
(2,5)  node[blue] (14)  {b}
(4,5)  node[blue] (15)  {c}
(4,6)  node[blue] (16)  {d}
(-3, 5)  node[blue] (17)  {f}
(-3,6)  node[blue] (18)  {g}
(-1, 6)  node[blue] (19)  {h}
(0, 9)  node[blue] (20)  {q}
(1,6)  node[blue] (21)  {i}
(1,7)  node[blue] (22)  {j}
(-5, 7)  node[blue] (23)  {k}
(-3, 7)  node[blue] (24)  {l}
(-1, 7)  node[blue] (25)  {m}
(-1, 8)  node[blue] (26)  {n}
(2, 7)  node[blue] (27)  {o}
(2,8)  node[blue] (28)  {e}
(2,10)  node[blue] (29)  {p}
(4, 9)  node[blue] (30)  {r}
(4, 10)  node[blue] (31)  {s}
(4, 12)  node[blue] (32)  {t}
(2, 13)  node[blue] (33)  {u}
(2, 12)  node[blue] (34)  {v}



;

%%rendezes a file elejere lett szamuzve

\end{tikzpicture}


